Temporal and Aspectual Entailment

Inferences regarding "Jane's arrival in London" from predications such as "Jane is going to London" or "Jane has gone to London" depend on tense and aspect of the predications. Tense determines the temporal location of the predication in the past, present or future of the time of utterance. The aspectual auxiliaries on the other hand specify the internal constituency of the event, i.e. whether the event of "going to London" is completed and whether its consequences hold at that time or not. While tense and aspect are among the most important factors for determining natural language inference, there has been very little work to show whether modern NLP models capture these semantic concepts. In this paper we propose a novel entailment dataset and analyse the ability of a range of recently proposed NLP models to perform inference on temporal predications. We show that the models encode a substantial amount of morphosyntactic information relating to tense and aspect, but fail to model inferences that require reasoning with these semantic properties.

==> _tables/agreement_results.tex <==
\begin{table}[!htb]
\centering
\small
\resizebox{0.65\columnwidth}{!}{
\begin{tabular}{ r | c c c c | c}
\textbf{Auxiliary}	& \textbf{\APT}		& \textbf{ELMo (+C)}		& \textbf{BERT}		& \textbf{\texttt{word2vec}}& \textbf{Majority Class}	\\\hline 
is 			& $0.88$ 			& $0.65$ $(0.63)$ 		& $\textbf{0.92}$ 	& $0.67$			& $0.67$ 			\\
will 			& $0.91$ 			& $0.66$ $\textbf{(0.94)}$ & $0.89$ 			& $0.67$			& $0.67$ 			\\
has 			& $\textbf{0.94}$ 	& $0.66$ $(0.63)$ 		& $0.90$ 			& $0.67$			& $0.67$ 			\\
had 			& $\textbf{0.94}$ 	& $0.66$ $(0.63)$ 		& $0.92$ 			& $0.67$ 			& $0.67$ 			\\
was 			& $0.83$			& $0.66$ $(0.64)$ 		& $\textbf{0.93}$ 	& $0.66$			& $0.67$ 			\\\hline
\textbf{Average} 	& $0.90$			& $0.66$ $(0.69)$ 		& $\textbf{0.91}$ 	& $0.67$			& $0.67$ 			\\
\end{tabular}}
\captionsetup{font=small}
\caption{Auxiliary-verb agreeement results.}
\label{tbl:agreement_results}
\end{table}

==> _tables/agreement_results_context.tex <==
\begin{table}[!htb]
\centering
\small
%\resizebox{\columnwidth}{!}{
\begin{tabular}{ r | c c c c c}
\textbf{Aux} & \textbf{ELMo} & \textbf{ELMo+C} \\\hline % ORDER 1 APTs INTERSECT \textbf{\APT} \\ \hline
is & $0.65$ & $0.63$  \\
will & $0.66$ & $0.94$  \\
has & $0.66$ & $0.63$  \\
had & $0.66$ & $0.63$  \\
was & $0.66$ & $0.64$  \\\hline
\textbf{Avg} & $0.66$ & $0.69$ 
\end{tabular}%}
\captionsetup{font=small}
\caption{AGREEMENT CLASSIFIER RESULTS.}
\label{tbl:agreement_results_context}
\end{table}

==> _tables/qualitative_analysis.tex <==
\begin{table}[!htb]
\centering
\small
\resizebox{0.6\columnwidth}{!}{
\begin{tabular}{ r | c c c c}
\textbf{Predication Pair} 			& \textbf{\APT} 	& \textbf{ELMo} 	& \textbf{BERT} 	& \textbf{\texttt{word2vec}}	\\\hline 
visit $\models$ leave				& $0.09$ 			& $0.59$ 			& $0.69$ 			& $0.36$ 			\\
is visiting $\models$ will leave 		& $0.02$ 			& $0.60$ 			& $\textbf{0.77}$ 	& $0.57$  			\\
is visiting $\not\models$ has left 	& $0.03$ 			& $0.65$ 			& $0.72$ 			& $0.58$  			\\\hline
visit $\models$ arrive 			& $0.07$			& $0.49$ 			& $0.71$ 			& $0.45$  			\\
is visiting $\models$ has arrived 	& $\textbf{0.04}$	& $\textbf{0.51}$ 	& $\textbf{0.84}$ 	& $\textbf{0.62}$  	\\
is visiting $\not\models$ will arrive 	& $0.01$			& $0.50$ 			& $0.81$ 			& $0.57$  			\\\hline
win $\models$ play 				& $0.14$ 			& $0.59$ 			& $0.73$ 			& $0.52$  			\\
has won $\models$ has played 		& $\textbf{0.25}$ 	& $\textbf{0.60}$ 	& $\textbf{0.85}$ 	& $\textbf{0.75}$  	\\
had won $\not\models$ will play 	& $0.11$ 			& $0.55$ 			& $0.78$ 			& $0.60$  			\\\hline
\end{tabular}}
\captionsetup{font=small}
\caption{Similarity scores between example predications.}
\label{tbl:qualitative_analysis}
\end{table}

==> _tables/tea_results.tex <==
\begin{table}[!htb]
\centering
\small
\resizebox{0.75\columnwidth}{!}{
\begin{tabular}{ r | c c c c | c}
\textbf{Similarity}	& \textbf{\APT}	& \textbf{ELMo}	& \textbf{BERT}		& \textbf{\texttt{word2vec}}	& \textbf{Majority class per Tense pair}\\\hline 
Cosine 			& $0.32$ 			& $0.28$ 		& $0.32$ 		& $0.33$ 			& $\textbf{0.37}$	\\
BInc / Classifier		& $0.30$ 			& $0.28$ 		& $0.22$ 		& $0.30$ 			& $\textbf{0.37}$	\\\hline
\end{tabular}}
\captionsetup{font=small}
\caption{Average precision scores on \textbf{TEA}.}
\label{tbl:tea_results}
\end{table}
